NASH: A Simple Unified Framework of Structured Pruning for Accelerating Encoder-Decoder Language Models

Structured pruning methods have proven effective in reducing the model size and accelerating inference speed in various network architectures such as Transformers. Despite the versatility of encoder-decoder models in numerous NLP tasks, the structured pruning methods on such models are relatively less explored compared to encoder-only models. In this study, we investigate the behavior of the structured pruning of the encoder-decoder models in the decoupled pruning perspective of the encoder and decoder component, respectively. Our findings highlight two insights: (1) the number of decoder layers is the dominant factor of inference speed, and (2) low sparsity in the pruned encoder network enhances generation quality. Motivated by these findings, we propose a simple and effective framework, NASH, that narrows the encoder and shortens the decoder networks of encoder-decoder models. Extensive experiments on diverse generation and inference tasks validate the effectiveness of our method in both speedup and output quality.

==> src/tab_component.tex <==
\begin{table}[t]
\centering
\caption{Component Analysis.}
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule[0.15em]
Task        & \multicolumn{2}{c|}{FLAN-T5 (SAMSum)} & \multicolumn{2}{c}{mT5 (OrangeSum)} \\ \midrule
& ROUGE-L & Speedup & ROUGE-L & Speedup \\ \midrule
Base      & 57.16 & 1.0$\times$ & 00.00 & 0.0$\times$ \\ \midrule
Small     & 51.42 & \textbf{3.1}$\times$ & 00.00 & 0.0$\times$  \\ 
CoFi-T5$^{*}$  & 41.82 & 1.8$\times$ & 00.00 & 0.0$\times$ \\ \midrule
\alg (2 decoder layers) & \textbf{52.09} & 2.5$\times$ & 00.00 & 0.0$\times$ \\
\alg (3 decoder layers) & 00.00 & 0.0$\times$ & 00.00 & 0.0$\times$ \\ \bottomrule
\end{tabular}
}\label{tab:component_analysis}
\end{table}

==> tex/99_intro_backup.tex <==
\section{Introduction}
% 첫 문단에서는 LLM을 먼저 간략하게 소개하면서 여러 성공이 있었다는 것을 이야기하고, Encoder, Decoder, Encoder-Decoder를 소개해주고, Encoder-Decoder가 가지는 장점을 이야기하고, translation, summarization에 특히 좋고 등을 이야기하면서 우리가 Encoder-Decoder에 관심을 가지고 있고 이게 중요한 구조이고 쓰임이 많은 구조이라는 것을 먼저 인지를 시키고,
In recent years, pre-trained language models (LMs) have demonstrated their effectiveness in various downstream tasks, such as natural language understanding (NLU) and natural language generation (NLG). Especially, there have been three main types of research, e.g., encoder-only LMs~\cite{devlin2019bert, he2023newmodel}, decoder-only LMs~\cite{touvron2023llama, openai2023gpt4}, and \textit{encoder-decoder} LMs~\cite{lewis-etal-2020-bart, raffel2020t5, chung2022flant5, tay2023ul2}, which aim for their specific expertise. However, these dramatic performances have demanded the necessity of huge computational and memory requirements. Therefore, it is necessary to develop computationally efficient, small-sized networks that can achieve comparable performance to that of larger models.

To reduce the significant computational costs, extensive research has been conducted on model compression methods. Among the various model compression techniques~\cite{jiao-etal-2020-tinybert, yao2022zeroquant}, pruning~\cite{frankle2018lottery, sanh2020movement, wang-etal-2020-strpruning_L0, xia-etal-2022-CoFi} is a promising method that aims to remove redundant weights from networks, resulting in improved efficiency by saving storage capacity and enhancing inference speed. In this paper, we specifically focus on structured pruning, which involves structured and unstructured approaches. Structured pruning is typically preferred in practice due to its relative ease of deployment on various types of hardware platforms compared to unstructured pruning~\cite{han-etal-2016-eie, Gupta2020CompressionOD}. % , kwon2022fast

\iffalse
In recent years, pre-trained language models (LMs) have demonstrated their effectiveness in various downstream tasks. These models can be broadly categorized into three types: encoder-only LMs~\cite{devlin2019bert, he2023newmodel}, decoder-only LMs, and \textit{encoder-decoder} LMs. While the recent success of decoder-only LMs~\cite{touvron2023llama, openai2023gpt4}, their achievements mainly stem from their large number of parameters, making them less accessible to the public. Additionally, smaller decoder-only LMs~\cite{radford2019language} showed limitations in tasks that contain important contextual information, such as natural language understanding (NLU) or summarization. In contrast, \textit{encoder-decoder} LMs~\cite{lewis-etal-2020-bart, raffel2020t5, chung2022flant5, tay2023ul2} have demonstrated their generality, allowing for their application across different network sizes and tasks ranging from NLU to various natural language generation (NLG), including translation and summarization.
% This versatility of encoder-decoder LMs has led to their widespread utilization~\cite{wang2023codet5+}, highlighting their importance in research and practical applications.

% 하지만 LLM은 너무 많은 parameter로 많은 연산이 필요하고 등등,, 그래서 이것을 줄이려는 시도들이 많이 존재하고 이런 저런 방법들을 소개하고 근데 이러한 시도들은 다 연구에 필요한 연산의 한계로 아쉽게도 Encoder에만 집중되어 있다. 이렇게 model compression의 중요성을 언급하면서 앞에서 강조한 Encoder-Decoder에 연구가 부족함을 상기시키고.
Despite the state-of-the-art performances of pre-trained LMs, their promising results come at the cost of significant computational and memory requirements.
% Consequently, deploying such large models on resource-constrained devices like mobile and wearable devices is impractical. 
Hence, there is a critical need to develop computationally efficient small-sized networks that can achieve comparable performance to that of larger models.
% This has motivated the development of model compression techniques, which can be categorized into pruning\,\cite{xia-etal-2022-CoFi}, knowledge distillation\,\cite{jiao2019tinybert}, and quantization\,\cite{yao2022zeroquant}, and we specifically focus on the pruning technique among them.
Among the various model compression techniques~\cite{jiao-etal-2020-tinybert, yao2022zeroquant} from such motivation, pruning~\cite{frankle2018lottery, sanh2020movement, wang-etal-2020-strpruning_L0, xia-etal-2022-CoFi} is a promising method that aims to remove redundant weights from networks, resulting in improved efficiency by saving storage capacity and enhancing inference speed. In this paper, we specifically focus on structured pruning which is typically preferred in practice due to its relative ease of deployment to various types of hardware platforms compared to unstructured pruning~\cite{han-etal-2016-eie, Gupta2020CompressionOD, kwon2022fast}.
\fi

% 본 연구에서는 Encoder-Decoder model에서의 structure pruning에 대한 연구를 진행한다고 선언을 하고. 앞에서 언급했던 여러가지 network compression 방법 중에서 굳이 이 방법을 중요하게 생각하고 연구하게 된 것인지를 잘 설명하기.
% In this paper, we focus on structured pruning which is typically preferred in practice due to its relative ease of deployment to various types of hardware platforms compared to unstructured pruning~\cite{han-etal-2016-eie, Gupta2020CompressionOD, kwon2022fast}.

While structured pruning, especially recent gradual methods~\cite{louizos2018l0_reg_prune, lagunas-etal-2021-block}, has shown effectiveness in pre-trained LMs, the existing literature primarily focuses on encoder-only LMs that are predominantly used for tasks such as sentiment analysis. Additionally, we found that when one of the state-of-the-art encoder-only methods, CoFi~\cite{xia-etal-2022-CoFi}, is directly applied to the encoder-decoder task, it exhibits a maximum speedup improvement of $1.53\times$ on the CNN/DailyMail~\cite{see-etal-2017-get} dataset with a ROUGE-L drop of $7.36\%$. This gain is considerably lower compared to the original result achieved on the encoder-only model applied to the worst QQP case in the GLUE dataset, where the speedup reaches $11.0\times$ with an accuracy drop of $1.20\%$. Therefore, it is necessary to investigate structured pruning methods specifically designed for encoder-decoder LMs.


% While structured pruning, especially recent gradual methods~\cite{louizos2018l0_reg_prune, lagunas-etal-2021-block}, has shown effectiveness in pre-trained LMs, the existing literature primarily focuses on encoder-only LMs used predominantly for tasks such as sentiment analysis. In addition, we verify that when one of the SoTA encoder-only method, CoFi~\cite{xia-etal-2022-CoFi} is directly applied to the \textit{encoder-decoder} task, it exhibits at most speedup improvement of $1.53\times$ on the CNN/DailyMail~\cite{see-etal-2017-get} with $7.36\%$ of ROUGE-L drop. This gain is considerably lower compared to the original result on the encoder-only model applied to the worst QQP case in the GLUE, where the speedup reaches $11.0\times$ with $1.20\%$ of accuracy drop. Therefore, investigating structured pruning methods for \textit{encoder-decoder} LMs is required.
% Furthermore, we check that when we apply the previous SOTA algorithm on encoder-only pruning method, CoFi, to the encoder-decoder model directly, the speedup gain of the encoder-decoder on SAMSum is $1.45\times$ which is significantly low compared to the encoder-only on the worst QQP case of GLUE benchmark, \emph{i.e.,} $11.0\times$.
% This biased research highlights on encoder-only rather than the others hampers 
% This research gap between encoder-only and the others


% Such research trend hampers the application of structured pruning in NLG tasks which entails significant computational costs due to the autoregressive decoding process that necessitates efficient computation. 
% Due to the disparity between \textit{encoder-decoder} and encoder-only LMs, in this paper, we ask: 
% (1) Can the method designed for \textit{encoder-only} LMs be directly applied to \textit{encoder-decoder} LMs? 

To this end, in this paper, we pose the following question: How can we design a structured pruning method that effectively accelerates the \textit{encoder-decoder} model while maintaining its performance? To the best of our knowledge, this study represents the first attempt to address this question. In order to accomplish this, we conduct systematic studies to examine the impact of structured pruning on the encoder and decoder networks, respectively.
% To the best of our knowledge, this is the first trial to answer this question based on the systematical studies on the perspective of the decoupled encoder and decoder pruning.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.82\linewidth]{fig/concept_figure.pdf}
    \caption{Brief illustration of the proposed algorithm, \alg. It is composed of two main components, width and depth pruning for encoder and decoder, respectively. }
    % This different type of pruning for each component is based on the empirical studies described in Section~\ref{sec:motivation}.
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}

% \vspace{-10pt}
\paragraph{Contribution.}
% \noindent
% \textbf{Contribution.\,}
In this study, we propose an algorithm called \alg, which is strongly motivated by two key findings derived from our preliminary experiments.
% s: (1) we observe the directly applying CoFi, which is one of the SOTA pruning methods for \textit{encoder-only}, to the \textit{encoder-decoder} model shows restricted efficiency gain $XX\%$ on the T5~\cite{raffel2020t5} compared to $XX\%$ on the BERT. Shortly speaking, this is because the previous approach fails to accomplish the target sparsity in the decoder. Detailed experimental settings and results are described in Appendix. (2) 
(1) \textbf{The number of decoder layers} is the primary factor influencing the speedup of inference. (2) \textbf{The sparsity of the encoder network} is a crucial factor affecting the output quality of \textit{encoder-decoder} models.

% To reduce the computation cost for \textit{encoder-decoder} models, we obtain two dominant factors: .

Based on these findings, we propose an algorithm, illustrated in~\autoref{fig:intro}, that consists of two parts: the encoder network, which enhances output quality by gradually reducing the width of each layer, and the decoder network, which achieves faster inference speed by uniformly selecting layers to reduce depth.

% The proposed algorithm mainly have two distinct parts: encoder network enhances output quality by gradually pruning via reducing the width of each layer, and decoder network is significantly pruned by uniformly selecting among the entire layers to accelerate inference speed. 
% The proposed algorithm aims to enhance output quality by gradually pruning the encoder network, while significantly pruning the decoder network using uniform layer selection to accelerate inference speed. 

We empirically evaluate the performance of \alg on various NLG datasets, including SAMSum~\cite{gliwa-etal-2019-samsum} and CNN/DailyMail, as well as NLU datasets~\cite{wang-etal-2018-glue, wang2019superglue}. Notably, in our experiments on NLG datasets using T5-base, \alg achieves a speedup of $2.5$-$4.2\times$ while preserving $95\%$ of the quality performance.
% Furthermore, we obtains $XX\%$ and $YY$ performance gains on GLUE and SuperGLUE compared to the XXX task.

% From the experiments, we observe that the proposed algorithm obtains $XX\%$ speedup with $YY\%$ performance degradation. It is $XX\%$ faster with small amount of $YY\%$ performance lose. 


% NLP task structured pruning 잘되었다.

% Existing literature on structured pruning of PLMs predominantly focuses on encoder-only models that are primarily used for NLU tasks like sentiment analysis and natural language inference. 

% This research gap hampers the application of structured pruning in NLG tasks which entail significant computational costs due to the autoregressive decoding process that necessitates efficient computation.

% 응 마지막에 한문단 더 이 문제가 왜 재밌는 문제이고 단순한 확장이 아닌지도 설명해주는게 좋을 것 같음
% Although structured pruning methods\,\cite{lagunas-etal-2021-block, xia-etal-2022-CoFi} have been widely applied to PLMs with high sparsity and speedup recently, they are still limited to the encoder-only models. Due to the disparity between \textit{encoder-decoder} and BERT-like LMs, in this paper, we ask: (1) Can the same method be applied successfully to \textit{encoder-decoder} LMs? (2) How can we develop the structured pruning method to speed up \textit{encoder-decoder} generative models? To the best of our knowledge, we are the first work to tackle this question and investigate the generality and feasibility of high-level sparsity structured pruning of generative models.

\iffalse
\paragraph{Contributions.} 
In this study, we conduct a systematic study to explore the feasibility and generality of structured pruning, specifically in the context of \textit{encoder-decoder} LMs.
We discover that achieving stable reductions in the depth of the decoder network and the width of the encoder network is vital for boosting inference speed without incurring significant performance drops~(\autoref{fig:finding_2}). Building upon these insights, we propose a novel pruning framework called \alg~(\textbf{NA}rrow encoder and \textbf{SH}allow decoder) that uniformly selects the decoder network for inference speedup and applies slight pruning to the encoder network to enhance generalization. Our extensive experimental results demonstrate that \alg achieves superiority in both inference speed and generation quality.
\fi

% It is important to emphasize that we first represent the difficulty of the previous structured pruning method for encoder-only LMs in \textit{encoder-decoder} LMs through our comprehensive investigation.
% To achieve faster inference speed, we propose a more stable and efficient approach by replacing the learning-based structural pruning of the decoder network with a uniform layer selection.
% Through our ablation studies, we verify the meaningfulness and effectiveness of each component in our proposed method, highlighting the careful design considerations involved, despite its simplicity.



% It is important to emphasize that we first represent the difficulty of the previous structured pruning method for encoder-only LMs in \textit{encoder-decoder} LMs through our comprehensive investigation.
% In our pursuit of achieving higher inference speedup, we have made a significant departure by replacing the structured pruning of the decoder network with a more stable and efficient uniform layer selection. 
% Through our ablation studies, we verify the meaningfulness and effectiveness of each component within our proposed method, demonstrating careful design considerations despite its simplicity.

% It is worth noting that we first identify the infeasibility of which are widely used in encoder-only models through our systematic study. To achieve higher inference speedup, instead, we simply replace the structured pruning of the decoder network with a uniform layer selection which is more stable, based on our main finding that the number of decoder network is primary factors for inference speed. Through our ablation studies, we validate the meaningfulness and effectiveness of each component within our proposed method, highlighting the careful design considerations made despite their simplicity.
